Evaluating Code Metrics in GitHub Repositories Related to Fake News and Misinformation

The surge of research on fake news and misinformation in the aftermath of the 2016 election has led to a significant increase in publicly available source code repositories. Our study aims to systematically analyze and evaluate the most relevant repositories and their Python source code in this area to improve awareness, quality, and understanding of these resources within the research community. Additionally, our work aims to measure the quality and complexity metrics of these repositories and identify their fundamental features to aid researchers in advancing the fields knowledge in understanding and preventing the spread of misinformation on social media. As a result, we found that more popular fake news repositories and associated papers with higher citation counts tend to have more maintainable code measures, more complex code paths, a larger number of lines of code, a higher Halstead effort, and fewer comments.

==> Research_goal_and_questions.tex <==
\subsection{Research Goal} 

Our research goal is to identify measures of code quality and complexity that may be associated with more popular fake news research or more popular fake news code repositories. This will ideally give researchers insight into the aspects of their research and shared code that are more associated with highly cited research or are valued by github users.
 
\subsection{Research Questions} 

RQ1:Is there any relationship between different measures of code metrics and the citations of the research?\\

 The main motivation of this research is to determine if there are any identifiable measures we can extract from the source code repository that is associated with the citations of a paper for that repository. We will identify common measures of code characteristics, quality, and complexity and check for correlation with related paper citations. This of course doesn't imply causality but will hopefully give insight into valued aspects of shared research and source code.
 
RQ2:Is there any association between different measures of code metrics and the github measures of popularity (stars and subs) ?\\ 

Same as RQ1 except with respect to the repository-specific measures of popularity like github stars and subscribers. We can see these are only loosely correlated with citations and we expect different measures to be associated with the repository popularity vs paper citations. Github measure like stars are selected by github users and arise from a very different process than paper citations. They could be subject to both manipulation or being ignored thus we'd expect them to be noisier indicators of popularity than citations. 

RQ3: Are there any code metrics that are associated with both GitHub measures of popularity and associated paper citations? \\ 
What we hope to answer with this question is whether are there any standard metrics or themes that  relate to the popularity of the repository across all of GitHub stars, followers, and paper citations. Because github measures and citations are somewhat orthogonal yet ostensibly both represent the popularity of the reseaarch and underlying code, we would hope to see some common factors underlying all of the measures. 

==> data.tex <==
%Methodology
\subsection{Github repositories} 
% Our primary goal in retrieving repositories is to find those are specifically related to fake news identification models with associated published, submitted or presented papers. To retrieve the repositories we're interested in,  we start out by searching GitHub for all repositories with the term "fake news" or misinformation after the date 1 Jan 2019 that have 2 or more subscribers and are greater than 1MB in size. We arrived at these criteria through trial and error trying to balance including as many candidates as possible while excluding  as many small tests, class assignments, and other meaningless repositories that would use up our valuable API request limits and slow down development. These criteria resulted in 414 (for 'fake news') and 64 (for misinformation) candidate repositories from which we further limited our analysis by requesting various attributes from GitHub and eliminating those that didn't represent a model-related research project. To do this we started off by eliminating anything that had an associated URL that contained  .ai, .io ,.guru, .br, .Br or flask, all of which we observed represented a demo application or more advanced class or resume-building project. After eliminating those we then included any project that any other associated URL, which was always associated with a link to a paper or research site, then include any repository that mentioned 'paper' 'conference' or 'proceedings in either the GitHub description or the README.md file. We also required the presence of at least one .py file in the repository to analyze. We also manually excluded a few different repositories which caused the third-party libraries to crash while parsing the python code, primarily python 2.7 and earlier code.
% We initially anticipated building a manual list of repositories to analyze but found some simple inclusion/exclusion criteria to be sufficient and robust enough to allow us to pick up new repositories and vary our date range, as our API limits allowed us to support many more samples than manually maintaining a list would allow. Table \ref{GitHub_repo_list} lists all the repositories and associated links we have considered in our analysis. It also has the corresponding followers, stars, and the creation time of those repositories. 



% % ...
% %\usepackage{graphics}
% \begin{table}[]
% \caption{Fake news related repositories retrieved from GitHub}
% \label{GitHub_repo_list}
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{|lllll|}
% \hline
% \multicolumn{5}{|l|}{\begin{tabular}[c]{@{}l@{}}Search Criteria: {[}repositories = \\ g.search\_repositories(query='fake news created:\\ 2020-01-01..* followers:\textgreater{}=3 size:\textgreater{}=1000'){]}\end{tabular}}                                                              \\ \hline
% \multicolumn{1}{|l|}{Repository url}                                                                                                                                                & \multicolumn{1}{l|}{Stars} & \multicolumn{1}{l|}{Subscribers} & \multicolumn{1}{l|}{Creation date}    & Creation time  \\ \hline
% \multicolumn{1}{|l|}{https://github.com/StanGirard/TrollHunter}                                                                                                               & \multicolumn{1}{l|}{39}    & \multicolumn{1}{l|}{4}           & \multicolumn{1}{l|}{2022-12-05} & 20:19:20 \\ \hline
% \multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}https://github.com/danielvegamyhre/\\ is-this-fake-news\end{tabular}}                                                         & \multicolumn{1}{l|}{29}    & \multicolumn{1}{l|}{1}           & \multicolumn{1}{l|}{2022-09-25} & 18:23:10 \\ \hline
% \multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}https://github.com/GitTeaching/\\ Fake-News-Detector-App\end{tabular}}                                                        & \multicolumn{1}{l|}{8}     & \multicolumn{1}{l|}{0}           & \multicolumn{1}{l|}{2022-11-04} & 5:29:40  \\ \hline
% \multicolumn{1}{|l|}{https://github.com/shiivangii/SpotFake}                                                                                                                  & \multicolumn{1}{l|}{21}    & \multicolumn{1}{l|}{1}           & \multicolumn{1}{l|}{2022-11-30} & 13:28:30 \\ \hline
% \multicolumn{1}{|l|}{https://github.com/nguyenvanhoang7398/FANG}                                                                                                              & \multicolumn{1}{l|}{56}    & \multicolumn{1}{l|}{2}           & \multicolumn{1}{l|}{2022-12-11} & 12:29:38 \\ \hline
% \multicolumn{1}{|l|}{https://github.com/fangyiyu/Fake\_News\_Detection}                                                                                                       & \multicolumn{1}{l|}{9}     & \multicolumn{1}{l|}{2}           & \multicolumn{1}{l|}{2022-11-29} & 17:50:42 \\ \hline
% \multicolumn{1}{|l|}{https://github.com/kennqiang/MDFEND-Weibo21}                                                                                                             & \multicolumn{1}{l|}{37}    & \multicolumn{1}{l|}{3}           & \multicolumn{1}{l|}{2022-11-28} & 15:09:53 \\ \hline
% \multicolumn{1}{|l|}{https://github.com/derevirn/gfn-detector}                                                                                                                & \multicolumn{1}{l|}{11}    & \multicolumn{1}{l|}{1}           & \multicolumn{1}{l|}{2022-03-06} & 4:48:13  \\ \hline
% \multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}https://github.com/GitHubLuCheng/Causal-\\ Understanding-of-Fake-News-Dissemination\end{tabular}}                             & \multicolumn{1}{l|}{18}    & \multicolumn{1}{l|}{1}           & \multicolumn{1}{l|}{2022-09-08} & 6:37:22  \\ \hline
% \multicolumn{1}{|l|}{https://github.com/RMSnow/WWW2021}                                                                                                                       & \multicolumn{1}{l|}{43}    & \multicolumn{1}{l|}{2}           & \multicolumn{1}{l|}{2022-12-04} & 10:45:22 \\ \hline
% \multicolumn{1}{|l|}{https://github.com/RMSnow/WWW2021}                                                                                                                       & \multicolumn{1}{l|}{43}    & \multicolumn{1}{l|}{2}           & \multicolumn{1}{l|}{2022-12-04} & 10:45:22 \\ \hline
% \multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}https://github.com/mandar196/\\ Fake\_News\_Classifier\_NLP\end{tabular}}                                                     & \multicolumn{1}{l|}{4}     & \multicolumn{1}{l|}{1}           & \multicolumn{1}{l|}{2022-08-10} & 16:42:44 \\ \hline
% \multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}https://github.com/AyushGupta51379/\\ COMP\_5331\_Project\_Fake\_News\_Detection\end{tabular}}                                & \multicolumn{1}{l|}{7}     & \multicolumn{1}{l|}{2}           & \multicolumn{1}{l|}{2022-12-02} & 16:05:29 \\ \hline
% \multicolumn{1}{|l|}{https://github.com/Nicozwy/CofCED}                                                                                                                       & \multicolumn{1}{l|}{33}    & \multicolumn{1}{l|}{3}           & \multicolumn{1}{l|}{2022-12-07} & 12:35:53 \\ \hline
% \multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}https://github.com/SauravMaheshkar/\\ Fake-News-Classification\end{tabular}}                                                  & \multicolumn{1}{l|}{8}     & \multicolumn{1}{l|}{1}           & \multicolumn{1}{l|}{2022-09-06} & 1:08:56  \\ \hline
% \multicolumn{1}{|l|}{https://github.com/mahithabsl/Fake\_News\_Detector}                                                                                                      & \multicolumn{1}{l|}{6}     & \multicolumn{1}{l|}{2}           & \multicolumn{1}{l|}{2021-12-02} & 18:59:55 \\ \hline
% \multicolumn{1}{|l|}{https://github.com/nguyenvo09/EMNLP2020}                                                                                                                 & \multicolumn{1}{l|}{55}    & \multicolumn{1}{l|}{1}           & \multicolumn{1}{l|}{2022-12-09} & 18:35:45 \\ \hline
% \multicolumn{1}{|l|}{https://github.com/nguyenvo09/EMNLP2020}                                                                                                                 & \multicolumn{1}{l|}{55}    & \multicolumn{1}{l|}{1}           & \multicolumn{1}{l|}{2022-12-09} & 18:35:45 \\ \hline
% \multicolumn{1}{|l|}{https://github.com/shaanchandra/SAFER}                                                                                                                   & \multicolumn{1}{l|}{14}    & \multicolumn{1}{l|}{3}           & \multicolumn{1}{l|}{2022-09-30} & 9:13:42  \\ \hline
% \multicolumn{1}{|l|}{https://github.com/shaanchandra/SAFER}                                                                                                                   & \multicolumn{1}{l|}{14}    & \multicolumn{1}{l|}{3}           & \multicolumn{1}{l|}{2022-09-30} & 9:13:42  \\ \hline
% \multicolumn{1}{|l|}{https://github.com/ICTMCG/Pref-FEND}                                                                                                                     & \multicolumn{1}{l|}{20}    & \multicolumn{1}{l|}{4}           & \multicolumn{1}{l|}{2022-12-11} & 8:19:07  \\ \hline
% \multicolumn{1}{|l|}{https://github.com/nguyenvo09/EACL2021}                                                                                                                  & \multicolumn{1}{l|}{32}    & \multicolumn{1}{l|}{2}           & \multicolumn{1}{l|}{2022-12-11} & 12:30:06 \\ \hline
% \multicolumn{1}{|l|}{https://github.com/nguyenvo09/EACL2021}                                                                                                                  & \multicolumn{1}{l|}{32}    & \multicolumn{1}{l|}{2}           & \multicolumn{1}{l|}{2022-12-11} & 12:30:06 \\ \hline
% \multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}https://github.com/hockeybro12/\\ FakeNews\_Inference\_Operators\end{tabular}}                                                & \multicolumn{1}{l|}{5}     & \multicolumn{1}{l|}{3}           & \multicolumn{1}{l|}{2022-12-07} & 16:27:48 \\ \hline
% \multicolumn{1}{|l|}{https://github.com/nermine-ali/Fake-news-detector}                                                                                                       & \multicolumn{1}{l|}{4}     & \multicolumn{1}{l|}{1}           & \multicolumn{1}{l|}{2020-03-27} & 15:09:22 \\ \hline
% \multicolumn{1}{|l|}{https://github.com/xiaolan98/BDANN-IJCNN2020}                                                                                                            & \multicolumn{1}{l|}{16}    & \multicolumn{1}{l|}{2}           & \multicolumn{1}{l|}{2022-09-14} & 8:32:47  \\ \hline
% \multicolumn{1}{|l|}{https://github.com/spChalk/Fake-News-Detection}                                                                                                          & \multicolumn{1}{l|}{6}     & \multicolumn{1}{l|}{2}           & \multicolumn{1}{l|}{2022-09-30} & 15:27:36 \\ \hline
% \multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}https://github.com/bkolosk1/\\ Multilingual-Detection-of-Fake-News-\\ Spreaders-via-Sparse-Matrix-Factorization\end{tabular}} & \multicolumn{1}{l|}{3}     & \multicolumn{1}{l|}{1}           & \multicolumn{1}{l|}{2022-09-13} & 18:07:18 \\ \hline
% \multicolumn{1}{|l|}{https://github.com/factsforfriends/frontend}                                                                                                             & \multicolumn{1}{l|}{4}     & \multicolumn{1}{l|}{1}           & \multicolumn{1}{l|}{2020-07-05} & 10:31:23 \\ \hline
% \multicolumn{1}{|l|}{https://github.com/Am1r8/Fake-news-Detector}                                                                                                             & \multicolumn{1}{l|}{4}     & \multicolumn{1}{l|}{1}           & \multicolumn{1}{l|}{2022-12-05} & 2:09:41  \\ \hline
% \multicolumn{1}{|l|}{https://github.com/anasasilva/desinforma.me}                                                                                                             & \multicolumn{1}{l|}{4}     & \multicolumn{1}{l|}{1}           & \multicolumn{1}{l|}{2022-05-16} & 9:40:58  \\ \hline
% \multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}https://github.com/ashu9999/\\ COVID19-Fake-News-Detection-Classification\end{tabular}}                                       & \multicolumn{1}{l|}{5}     & \multicolumn{1}{l|}{2}           & \multicolumn{1}{l|}{2022-10-06} & 16:53:26 \\ \hline
% \multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}https://github.com/alooperalta/\\ Fake-News-Detection-System\end{tabular}}                                                    & \multicolumn{1}{l|}{4}     & \multicolumn{1}{l|}{1}           & \multicolumn{1}{l|}{2022-04-28} & 11:02:58 \\ \hline
% \multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}https://github.com/Bhavik-Jikadara/\\ Fakes-News-Detection\end{tabular}}                                                      & \multicolumn{1}{l|}{3}     & \multicolumn{1}{l|}{1}           & \multicolumn{1}{l|}{2022-12-10} & 10:52:18 \\ \hline
% \multicolumn{1}{|l|}{https://github.com/chiraag-kakar/FUND}                                                                                                                   & \multicolumn{1}{l|}{5}     & \multicolumn{1}{l|}{1}           & \multicolumn{1}{l|}{2021-05-10} & 17:53:40 \\ \hline
% \multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}https://github.com/JoykishanSharma/\\ Covid-19-Mobile-Updater-App\end{tabular}}                                               & \multicolumn{1}{l|}{3}     & \multicolumn{1}{l|}{2}           & \multicolumn{1}{l|}{2022-08-22} & 3:42:08  \\ \hline
% \multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}https://github.com/priyanshishah/\\ Multimodal-fakenews-detection\end{tabular}}                                               & \multicolumn{1}{l|}{5}     & \multicolumn{1}{l|}{1}           & \multicolumn{1}{l|}{2022-11-23} & 13:01:21 \\ \hline
% \multicolumn{1}{|l|}{https://github.com/JoaoEnrique/FactNews}                                                                                                                 & \multicolumn{1}{l|}{3}     & \multicolumn{1}{l|}{1}           & \multicolumn{1}{l|}{2022-02-10} & 18:27:04 \\ \hline
% \multicolumn{1}{|l|}{https://github.com/jurgen1c/CS-Media}                                                                                                                    & \multicolumn{1}{l|}{7}     & \multicolumn{1}{l|}{1}           & \multicolumn{1}{l|}{2021-03-28} & 19:46:37 \\ \hline
% \multicolumn{1}{|l|}{https://github.com/srinjoychakravarty/authentikos}                                                                                                       & \multicolumn{1}{l|}{4}     & \multicolumn{1}{l|}{1}           & \multicolumn{1}{l|}{2020-06-02} & 23:59:24 \\ \hline
% \multicolumn{1}{|l|}{https://github.com/rprokap/pset-9}                                                                                                                       & \multicolumn{1}{l|}{52}    & \multicolumn{1}{l|}{28}          & \multicolumn{1}{l|}{2022-12-07} & 20:18:09 \\ \hline
% \multicolumn{1}{|l|}{https://github.com/danderfer/Comp\_Sci\_Sem\_2}                                                                                                          & \multicolumn{1}{l|}{5}     & \multicolumn{1}{l|}{3}           & \multicolumn{1}{l|}{2022-12-10} & 19:20:30 \\ \hline
% \end{tabular}%
% }
% \end{table}


==> future.tex <==
For subsequent enhancement of this study, we would hope to expand and clean up our data set to allow us to use some more advanced models and statistics in analyzing the relationships. The generalization of our software to work with arbitrary search terms would be interesting in analyzing further research domains. Integrating a more sophisticated searching process for paper titles in order to use Google Scholar and Semantic Scholar python libraries to automatically gather citations would eliminate the manual aspect of our citation data gathering. Further normalization of the dataset variables would improve both the predictability and allow us to use some of the other high collinear variables which would have more orthogonality when normalized. We would love to add the ability in our code to switch between multiple GitHub API tokens when API limits are hit, speeding up data gathering and research. More sophisticated feature and model selection would be interesting to see if additional relationships arise from something different than the linear models used. In addition, we also plan to include specific python code quality tools to evaluate the fake news repositories.   

==> old_fakenews.tex <==
\subsection{Fake News Overview} 
The Web2.0 technology has accelerated the consumption of fake news in social media. In one instance, the middle schoolers at Philadelphia believed that the earth is flat because of the idea they picked up from basketball star Kyrie Irving, who said that on a podcast\cite{b1}.The instructors further reported that it is difficult to change a child’s misconceptions once they are exposed to misinformation  \cite{b1}. With the alarming rise of fake news, there is a compelling need for understanding the dynamics of misinformation in social media. 

Shu et al. \cite{b2} focus on considering a tri-relationship among user, publisher, and news content. User engagements represent the news proliferation process over time, which provides useful auxiliary information to infer the veracity of news articles. Shu et al. \cite{b3} have proposed a detection method using explicit and implicit features from data, which has the potential to differentiate fake news.

Jonathan Albrig \cite{b4} analyzed the role of Facebook in the election of 2016, the article also discussed the influence of hyper biased news over the search engine and all over the internet. The study claims that not only large social media advertisements are an emotional spread of the misinformation, but the algorithm amplifies it. The study also found that only 60\% of the misinformation source is a social media platform, the rest 40\% of the misinformation comes from the direct website. The study vastly discussed the Micro Propaganda Machine, which is an influence network, that can tailor users opinions, emotional reaction, and create a viral sharing.

In the paper \cite{b5},the authors Srijan Kumar and Neil Shah presented a comprehensive study of the actors, rationale, and impact of the successful spreading of false information, as well as its characteristics of it and its detection algorithm. They found the creation and spreading of false information are generally controlled by a single entity with synthetically created fake accounts following each other. The spreading rate of fake is very high, especially at the initial state, even before it is debunked. This paper’s survey found that generally, the text is longer, more exaggerated, repetitive, incoherent, and more opinionated in false news, created and spread in a short period of time from the same group of relatively new accounts of fewer reviews with overlapping local networks. Also, the”echo-chamber effect” (self-selective polarizing effect on the content of predetermined beliefs), or improved technologies like content personalization may cause the same kind of fake news to come up several times and make people believe it. However, several algorithms Feature-based, Graph-based, Propagation-modeling based have been created for operative detection of false information. 

\par Horne and Adali enlisted that \cite{b6}, (f1) fake news articles tend to be shorter in terms of content but use repetitive language, smaller words, less punctuation, and fewer quotes. (f2) fake news articles require a lower educational level to read, use fewer analytic words, use more personal pronouns and adverbs, but fewer nouns. (f3) fake titles are longer, contain shorter words, use more capitalized words, fewer stop words, and fewer nouns overall but more proper nouns. (f4) titles are a strong differentiating factor between fake and real news. Anu et al. \cite{b7} reproduced the study by Horne and Adali and confirm most of the original paper’s findings regarding title and body feature differences between fake and real news. However,  differently from Horne and Adali, they found that fake titles contain more stop words, and, both titles and bodies express more negative emotions and sentiments than the real ones. Real news articles are more descriptive than fake news ones. Also, they highlight some differences between two different news domains: political and gossip. For instance, among stylistic, psychological, and complexity features in the news title, psychological features are the most important group of features for gossip news, while for political news it is the stylistic features. This shows how gossip news titles tend to be more persuasive than other news domains.

\par Anu et al. \cite{b8} found that News headlines are more informative than news body content, suggesting that we can avoid “read” the news excerpt and focus on other modalities to better detect misleading news. By comparing the news headline and excerpt content, the authors observe that headline characteristic are more consistent than excerpt ones across datasets. They also argued publisher bias is a strong predictor of news validity. In fact, by analyzing information collected from mediabiasfactcheck.com (“the most comprehensive media bias resource on the Internet”), they showed that hyper-partisan (extremely biased towards a political party) news sources are more likely to spread misleading stories than other sources.

\par Images in news articles also play a role in misleading news detection \cite{b9}. Fake images are used in news articles to provoke emotional responses from readers. Images are the most eye-catching type of content in the news; a reader can be convinced of a claim by just looking at the title of the news and the image. Jin et al. \cite{b10} showed that including visual and statistical features extracted from news images improves the results for microblogs news verification.

\par The paper \cite{b11},  focuses on news and media literacy and defines, explicates, and operationalizes news literacy combining it with the knowledge of news production, distribution, and consumption with five conceptualized domains. For The rationale and purpose of the definition of news literacy, authors firstly put emphasis on importance on knowledge and skill and secondly, discussed how news literacy should be defined and distinguished from related literacies. Authors came to a definition like, “ news literacy as knowledge of the personal and social processes by which news is produced, distributed, and consumed, and skills that allow users some control over these processes. Authors proposed five knowledge and skills domains – context, creation, content, circulation, and consumption, which make up the core of news literacy though empirically there are some overlaps between each of these domains. 
